Identifying the Major Sources of Variance in Transaction Latencies: Towards More Predictable Databases

Decades of research have sought to improve transaction processing performance and scalability in database management systems (DBMSs). However, significantly less attention has been dedicated to the predictability of performance: how often individual transactions exhibit execution latency far from the mean? Performance predictability is vital when transaction processing lies on the critical path of a complex enterprise software or an interactive web service, as well as in emerging database-as-a-service markets where customers contract for guaranteed levels of performance. In this paper, we take several steps towards achieving more predictable database systems. First, we propose a profiling framework called VProfiler that, given the source code of a DBMS, is able to identify the dominant sources of variance in transaction latency. VProfiler automatically instruments the DBMS source code to deconstruct the overall variance of transaction latencies into variances and covariances of the execution time of individual functions, which in turn provide insight into the root causes of variance. Second, we use VProfiler to analyze MySQL and Postgres - two of the most popular and complex open-source database systems. Our case studies reveal that the primary causes of variance in MySQL and Postgres are lock scheduling and centralized logging, respectively. Finally, based on VProfiler's findings, we further focus on remedying the performance variance of MySQL by (1) proposing a new lock scheduling algorithm, called Variance-Aware Transaction Scheduling (VATS), (2) enhancing the buffer pool replacement policy, and (3) identifying tuning parameters that can reduce variance significantly. Our experimental results show that our schemes reduce overall transaction latency variance by 37% on average (and up to 64%) without compromising throughput or mean latency.

==> case-study.tex <==
%!TEX root = predictability.tex

\section{Latency Variance in MySQL}
\label{sec:identification}

We use \vprofiler\ to characterize sources of latency variance in MySQL 5.6.23 when running the TPC-C benchmark
using OLTP-Bench~\cite{oltpbench} software suite.
We study two configurations.
First, we study a conventionally scaled 128-warehouse configuration with a 30 GB buffer pool on a system with 2 Intel(R) Xeon(R) CPU E5-2450 0 @ 2.10GHz cores. 
Second, we study a reduced-scale 2-warehouse configuration with a 128M buffer pool on a machine with 2 Intel Xeon E5-1670v2 2.5GHz virtual CPUs. 
The reduced scale configuration exaggerates buffer pool contention, revealing latency sources that arise when the buffer pool is too small to fit the working set.
In both cases, we use a separate client system to issue requests to the MySQL server.


Table \ref{tab:source} shows the main sources of variance we discovered using the \vprofiler\ framework for these configurations.
Note that the table reflects invocations of \texttt{os\_event\_wait} from two different call sites.

\begin{table}[h!]
\small
\centering
\begin{tabular}{|c|c|c|} \hline
Config&Function& \% Latency Var.\\ \hline
128-WH&\texttt{os\_event\_wait} [A] &37.5\%\\ \hline
128-WH&\texttt{os\_event\_wait} [B]&21.7\%\\ \hline
128-WH&\texttt{row\_ins\_clust\_index\_entry\_low}&9.3\%\\ \hline
2-WH&\texttt{buf\_pool\_mutex\_enter}&32.92\%\\ \hline
2-WH&\texttt{img\_btr\_cur\_search\_to\_nth\_level}&8.3\%\\ \hline
2-WH&\texttt{fil\_flush}&5\%\\
\hline\end{tabular}
\caption{Key Sources of Variance}
\label{tab:source}
\end{table}

\subsection{os\_event\_wait} 
MySQL includes its own cross-platform API for locks and condition variables; \texttt{os\_event\_wait} is one of the central functions in this abstraction layer. 
This function is similar to the platform-specific \texttt{pthread\_cond\_wait} function on Linux, which is used to wait on a conditional variable. 
This function is  used extensively for varied purposes, especially when MySQL executes under the serializable isolation level, wherein locking is the concurrency control mechanism. 
The implementation of \texttt{os\_event\_wait} yields little insight into why transaction execution is blocked.
Instead, we examine the context for the two most significant call sites that invoke \texttt{os\_event\_wait}.  Both the instances noted in the table arise in the execution of  \texttt{lock\_wait\_suspend\_thread}, which is used to put a thread to sleep when its associated transaction tries to acquire a lock on some data record, but must wait due to a lock conflict. 
These two specific instances correspond to locks acquired during select and update statements, respectively.

The implication of this result is that variability of wait time for contended locks is the largest source of variance in MySQL running TPC-C.  This finding motivates our study of variance-aware transaction scheduling, which seeks to optimize contended lock transfers to minimize wait time variance.

\subsection{row\_ins\_clust\_index\_entry\_low} 
The cluster index is a special kind of index in Innodb in which all row data is stored. 
Innodb reuses existing indexes as cluster indexes or creates new indexes when no appropriate index can be found. 
All other indexes are secondary indexes. 
The function \texttt{row\_ins\_clust\_index\_entry\_low} inserts a new data record into a cluster index, which is a critical step in the execution of insert operations.
None of the children of this function have sufficiently significant variation to be selected by \vprofiler's factor selection algorithm. The variance arises in the body of \texttt{row\_ins\_clust\_index\_entry\_low} due to varying code paths taken based on the state of the index prior to the insert operation.

\subsection{buf\_pool\_mutex\_enter}
The function \texttt{buf\_pool\_mutex\_enter} is called when other functions must access the buffer pool.
Like \texttt{os\_event\_wait}, it is called from various sites. 
This instance is called from \texttt{buf\_page\_make\_young}, which is used to move a page to the head of the list that manages buffer page replacements. 
InnoDB replaces buffer pool pages using a variant of the least recently used algorithm.
The buffer page replacement order is maintained in a list called \texttt{LRU}.  
Upon certain kinds of accesses, a page must be located and moved to the head of the \texttt{LRU} list. 
Threads must acquire a lock before accessing the LRU list; that lock is acquired in \texttt{buf\_pool\_mutex\_enter}. 
The variance in this function reflects waiting time while other threads execute \texttt{buf\_page\_make\_young} to reorder the LRU list.

\subsection{btr\_cur\_search\_to\_nth\_level}
\texttt{btr\_cur\_search\_to\_nth\_level} traverses an index tree, placing a tree cursor at a given level and leaving a shared or exclusive lock on the cursor page. 
A performance-critical loop in this function traverses from level to level  in the index tree, and its runtime varies with the depth to which the tree must be traversed.  
The variance we observe in this function is inherently due to the index traversal, not a performance pathology.

\subsection{fil\_flush}
In operating systems that use disk buffering to improve I/O performance, the \texttt{fil\_flush}  function performs a flush operation on the redo logs generated during the execution of a transaction. When disk buffering is enabled, this function becomes the one executing the I/O operations, instead of the \texttt{write} system call. 
The variance in of this function, is therefore due to the variance in I/O operations, which can be caused by different disk seek times or different data sizes flushed to disk.




